Efficient Compilation for Shuttling Trapped-Ion Machines via the Position Graph Architectural Abstraction

With the growth of quantum platforms for gate-based quantum computation, compilation holds a crucial role in deciding the success of the implementation. While there has been rich research in compilation techniques for the superconducting-qubit regime. The trapped-ion architectures, currently leading in robust quantum computations for their reliable operations, still lack competitive compilation strategies. This work introduces a unifying hardware abstraction, the ``position graph'', representing various hardware architectures. With this abstraction, we model trapped-ion Quantum Charge-Coupled Device (QCCD) architectures, enabling high-quality, scalable compilation methods. Specifically, we propose scheduling algorithms called SHuttling-Aware PERmutative (SHAPER) and SHuttling-AWare (SHAW) heuristic searches to tackle the complex constraints and dynamics of trapped-ion machines, with the cooperation of state-of-the-art permutation-aware mapping. These approaches generate executable circuits and native instructions that respect the physical constraints of shuttling-based architectures. We evaluate proposed algorithms across theorized and real architectures using the position graph framework. For completeness, we also introduce a linear program of trapped-ion scheduling that yields the optimal schedules, enabling a direct comparison with our heuristics. Our algorithm can successfully compile programs for extreme architectures where priori algorithms fail. When the baseline does complete, our produced schedules are $1.45$ times faster on average, with best-case speedups up to $4$ times faster.

==> isca2024/content/rebuttal_letter.tex <==
\newpage
\section*{Author's response letter}
Dear Reviewers and Editors,

We express our gratitude to all reviewers for their time and effort. The comments are absolutely invaluable and helped to improve the paper. We first respond to the joint concern about the scalability and then address other questions raised by individual reviewers in paragraphs right after the quotes of the comments. In this revision, we have implemented many modifications and clarifications that enhance the quality of the manuscript according to the reviews.
% Furthermore, the first author realized a mistake when evaluating the performance of SHAPER/SHAW and QCCDSim in Table \ref{tab:small-circuit} (wrong gate execution time), which has been fixed in the latest manuscript. 

New content has been highlighted in \color{blue} Blue \color{black} in the revised manuscript for easy identification.

\paragraph{\textbf{Question about the scalability of the proposed algorithms on larger architectures [Reviewers~1,~2]}}
We address the concern about the scalability of the proposed method by running both SHAPER/SHAW on the larger architectures. We continue to use ``grid'' architecture to show the result when scaling up to a $128$-qubit circuit. The result is shown in Table \ref{tab:full-result-large-scale}.

It is very illuminating that we observe that for larger experiments, QCCDSim runtime scales badly with the number of total ions in an architecture. By perform power law fitting model $y = a{x}^{b}$, where $x$ is the number of total ions, we can see that the exponent factor $b$ for both SHAPER and SHAW is around $3$, which is much better than QCCDSim, around $6$. Although the constant factor $a$ for SHAPER and SHAW is worse than QCCDSim, we emphasize that this constant factor can be due to the implementation and engineering factors. For the algorithm scaling factor $b$, SHAW and SHAPER show an improvement.

Besides the improvement in the algorithm scaling, both SHAPER and SHAW show a substantial improvement in performance compared to QCCDSim for large-scale instances. On average, SHAPER gives schedules with operation time that are $68\%$ faster, while SHAW gives a $70\%$ faster schedule than QCCDSim. This is a big improvement, especially for a large-scale circuit. Another interesting take is for $128$-qubit circuits, QCCDSim still fails when the total number of ions is $144$, which is $12.5\%$ more ions than the actual required number of ions.

We add another paragraph that discusses this large-scale result in Section \ref{sec:evaluation}

\subsection*{Reviewer 1 comments: }

\noindent\textbf{Novelty and potential for innovation:} \textit{``This work is inspired by the well-known SABRE yet introduces new features by targeting multi-trap architectures and exploiting two mechanisms to escape local minima and resolve congestion. Nonetheless, one potential concern is that the argument of novelty in the Introduction may appear overstated to readers. One of the specific sentences is “… first attempt to narrow the difference between different quantum architectures...”. First, several conditions exist in the class of hardware that the proposed compilers would newly support: (i) trapped-ion qubits, (ii) the all-to-all gate run within each trap, and (iii) the presence of T- or Y-junctions. Given these constraints, the scope of the claimed contribution may appear broader than what is demonstrated.
Recent related studies targeting trapped-ion systems exist. For example, arXiv:2207.01964v4 presents a compiler for architectures without all-to-all operations inside a trap, requiring ions to be repositioned into nearest-neighbor configurations before two-qubit gate runs. Muzzle the Shuttle (DATE ’22) considers processors with multiple traps and proposes optimizations that incorporate gate distances and nearest-neighbor trap interactions. Although it does not model the T- or Y-junction structures considered here, it still addresses compilation challenges in linearly connected multi-trap systems. The scope of novelty could be more precisely described as focusing on architectures where (i) all-to-all gate operations are supported within a trap and (ii) 2-D multi-trap topologies are possible via T- or Y-junctions. The authors may consider either expanding the discussion to address architectures beyond these scopes or revising their novelty claim.''}

$\rightarrow$ Thank you for raising this concern about the scope of the novelty. We do not want to overstate the scope of the novelty of our project; therefore, we have made  modifications in section \ref{sec:Intro} (Introduction) and clearly state that ``For QCCD-based TI architecture as defined in Section \ref{sec:QCCD}, we can use our abstraction to represent it, as well as the superconducting system as discussed in Section \ref{sec:sc_encoding}". Following your suggestions, we also expanded the discussion, which discusses the architectures beyond these scopes in Paragraph ``Potential unifying abstraction across architectures''.\\

\noindent \textbf{Soundness of the idea, and the methods and techniques proposed:} \textit{``The proposed methodologies are well-explained. Section 5 explains how arbitrary junction types (Y or T, Y+Y, X) are abstracted into the position-graph representation, and Section 6 provides a description of the SHAPER heuristic search algorithm.''}

$\rightarrow$ Thank you for your comment\\

\noindent \textit{``Nevertheless, one potential concern may be insufficient analysis or discussion of the overhead associated with additional gates inserted to reduce shuttling costs, as shown in Figure 2. The proposed approach appears to prioritize and maximize in-trap operations by introducing extra gates that help reduce inter-trap shuttling from a global execution perspective. Could the authors discuss the impact of these additional gates on fidelity degradation or increased circuit depth? Given that trapped-ion processors typically have very high single-qubit gate fidelities and long coherence times, inserting a small number of gates to reduce shuttling is likely a favorable tradeoff. A detailed discussion of the impact of the added gates on fidelity would strengthen the work.''}


$\rightarrow$ Thanks for this interesting comment. The main point of minimizing ions' shuttling time indeed is to minimize the circuit infidelity. To support this point, we add the fidelity model as shown in Section \ref{sec:exp_setup}, where we show how gate fidelity is affected by the heating introduced by shuttling. As commented by Reviewer~1, introducing more gates as in Figure \ref{fig:concrete_ex} can be harmful to overall fidelity. Here, we clarify that we have already considered this main objective in the synthesis process by examining both gate count and congestion objectives (potential for faster shuttling) during circuit synthesis (see Section \ref{sec:pam_map}). 

Furthermore, as QCCDSim does not support synthesis, we emphasize in the Section \ref{sec:exp_setup} that we already transpile all the circuits into native gatesets before the compilation with a strong BQSKIT compiler for fair comparison. We observed that due to this near-optimal compiled circuit, the added benefit of SHAPER's Permutation-aware synthesis is primarily in selecting permutations that provide better shuttling. In the case of SHAW, the heuristic did not have the Permutation-aware synthesis; therefore, its gate count does not change after the compilation. We clarify this fidelity objective in Section \ref{sec:exp_setup} and add this discussion in \textit{``Gate count overhead and Circuit fidelity''} in Section \ref{sec:exp_result}.\\

\noindent\textit{``Additionally, the proposed method relies on the Floyd–Warshall algorithm for finding the shortest path in the position graph, which scales as O($n^3$) in the number of nodes, n. As future QCCD architectures scale up, compilation costs may become a limiting factor.''}

$\rightarrow$ Thank you for raising a concern about the scaling of the Floyd–Warshall algorithm, where the time complexity $\mathcal{O}(V^{3})$ makes it a good choice for dense small graphs only. Alternatively, for a large and sparse graph, we propose using repeated Dijkstra's algorithm, where the time complexity is commonly known as $\mathcal{O}(V(V+E)\log(V))$, which can give an improvement against FW. Besides this, algorithms such as Johnson and $\mathrm{A}^{*}$ can also be considered, as those are generally faster for sparse graphs. Moreover, parallelism can also be used as in [(ASCE)CP.1943-5487.0000220]. We briefly discussed this when we first introduced the Floyd–Warshall algorithm in Section \ref{sec:our_algo}.\\

\noindent\textbf{Experimental evaluation: } \textit{``SHAPER and SHAW are evaluated across various NISQ programs. One potential concern is that the proposed approach may appear to trade substantial compilation time for relatively modest reductions in shuttling time. Given future QCCD development directions that scale up toward very large electrodes, the current compilation cost scalability may raise a potential concern about the realism of the proposed methodologies.
In Table 3, for the QV\_16 on the G2x3 with six traps and four ions/trap, SHAPER reduces the shuttling time by roughly 35\% compared to QCCDSim, but the compilation time increases by a factor of approximately 1025. In this case, SHAPER spends an additional 317 seconds of compilation to save approximately 3.5 milliseconds of shuttling time, compared to QCCDSim. While the reviewer understands that reducing shuttling overhead is indeed beneficial and required for currently available error-prone trapped-ion systems, it would be vital to quantitatively demonstrate how these reductions translate into meaningful improvements in fidelity.''}

$\rightarrow$ We thank the reviewer for such detailed comments. To deal with this concern about the scalability issue, we address this comment, as in the first part about the scalability concern ``\textbf{Question about the scalability of the proposed algorithms }''.\\

\noindent \textit{``For improving the depth of evaluation, the authors are recommended to include fidelity evaluations, which substantiate the advantages of their approach. As shown in Figure 2, the proposed method inserts extra gates to minimize shuttling costs. Based on the reviewer's understanding, adding extra gates may slightly degrade fidelity, but reducing shuttling is expected to improve overall fidelity. Could the authors include analyses of the combined fidelity impact of these two factors? For such fidelity estimates, it may be possible to reference hardware specifications from well-known commercial TI processors, such as those from IonQ or Quantinuum. Including this type of analysis would further strengthen the work.[$\dots$] Finally, additional experiments of compilation cost scalability under larger architectures would enhance the realism of the evaluation.''}

$\rightarrow$ Thank you for these comments. The gate count overhead is addressed in the comments above. Here, we take a deeper look into the circuit fidelity through Table \ref{tab:fidelity-circuit}. In the table, we calculate the circuit fidelity of configurations where SHAPER/SHAW and QCCDSim performance have a small gap. Interestingly, not all the cases where SHAPER/SHAW gives better shuttling time yield better fidelity. In the cases where we have a relatively big gap, such as for $8$-qubit circuits or $\geq 32$-qubit circuits, it is almost guaranteed to have the fidelity improvement (the motion introduced in Equation \ref{eq:gate_fidelity} kills the gate fidelity). As heating follows ions when merging into the trap and splitting out of the trap, as described when introducing the gate fidelity model in Section \ref{sec:exp_setup}, when having similar operation times, the circuit fidelity highly depends on the scheduling sequence. Therefore, for configurations with a small gap in operation time between our proposed method and QCCDSim, sometimes we beat it, and sometimes we lose when comparing the circuit fidelity. Nevertheless, this gives a very interesting point where the shuttling time is not sufficient, but the fidelity model also matters. We add this part to \textit{``Gate count overhead and Circuit fidelity''} in Section \ref{sec:exp_result} and the discussion \textit{``Better mapping algorithm based on the position graph abstraction''} in Section \ref{sec:discussion}


As the reviewer points out, using hardware specifications from well-known commercial TI processors can be a good addition. However, as the author can not find many details about the shuttling operation timing, heating model, and fidelity model of these commerical processors, we decide to stick with the well-known model deriving from real experiments in [PhysRevA.99.022330] \\


\noindent \textit{``Also, for strict comparison, adopting QPU's total runtime would be recommended, which includes shuttling time and gate application time. It would be helpful to quantify the total QPU runtime reduction achieved and to evaluate whether this reduction leads to fidelity gains.''} 

$\rightarrow$ Thank you for this wonderful comment. From the beginning, what we have been reporting was operation time ($\mu$s), which comprised gate execution time and ion shuttling time. We have fixed this in our manuscript. As the gate count is the same, we always have better fidelity than the benchmark.\\


\noindent \textit{``Explicitly explaining the evaluation setup for the native instruction set in Section 7.1 is also recommended.''}

$\rightarrow$ To address the comment about the native instruction set, we add a part that states the native gateset that we are using. Moreover, we add a reference to this timing setup. For large-circuit experiments, we use the timing as defined in the table, where details of the timing are added in the first part of Section \ref{sec:evaluation}.\\

\noindent\textbf{Presentation of the paper:}
\textit{``The topic in this work is timely and well-motivated. Compilation strategies are important for trapped-ion processors. The proposed position graph-based abstractions can model a range of trap architectures. Compared with superconducting qubits, trapped ions have much longer T1 times but slower gate application processes, and physical ion transport is required. Thus, developing compilation techniques that minimize shuttling is essential. Existing compilers tend to optimize programs independently of the machine and, for example, do not distinguish between long-range and short-range gates in the logical circuit, potentially leading to sub-optimal compilation results.''}

$\rightarrow$ Thank you for your comment \\

\noindent\textit{``Nevertheless, it is recommended that some descriptions of visual materials in the manuscript be rewritten to minimize redundancy and to be fully explained. If the reviewer’s understanding is correct, Fig. 4 (b) could be described as follows: (i) Each node in the graph represents a physically occupiable location where a qubit may reside. (ii) The circles with a black border abstract the available positions inside a trap. A position colored purple indicates that a qubit currently occupies that location, while a white circle indicates that the area is empty. (iii) The dotted black edges within each trap indicate pairs of positions between which a two-qubit gate operation is possible. (iv) The circles with a yellow border represent abstract intermediate positions where a qubit may temporarily reside while moving between traps. (v) The blue edges abstract the allowable relationship networks along which a qubit may temporarily move to reach another trap.''}

$\rightarrow$ Thank you for such a detailed comment. Your understanding of the position graph translation is totally correct, and it also gives us a very good suggestion to describe our abstraction better. We will gladly follow it to make it easier to understand. Based on your suggestion, we edited the caption of Figure \ref{fig:position_physical} for clarification.\\

\noindent \textbf{Reason to accept/reject:}\textit{\begin{itemize}
    \item The authors may consider revising the scope of the novelty claims in Section 1.
    \item It is recommended to include additional analyses and evaluations for depth and realism: total QPU runtime  (not only shuttling time), impact of fidelity drop according to introducing additional gates for minimizing shuttling, and computational complexity's scalability of the proposed algorithms for larger QCCD architectures.
    \item It would be beneficial to describe the native gate set in the evaluation setup.
\end{itemize}
}
$\rightarrow$ Thanks for all the concern that you have shown. These really help improve the manuscript by a lot. We hope all of our answers can satisfy your concern.

\subsection*{Reviewer 2 comments: }

\noindent \textbf{Soundness of the idea, and the methods and techniques proposed:}\textit{``The paper proposed SHARPER/SHAW, a scheduler and compiler for shuttling TI machines using the position graph as a intermediate representation. The graph captures the conflict/shuttling paths, but lacks detail explaination on how to convert a given device configuration to a certain position graph, and why the conversion is plausible.''}

$\rightarrow$ To clarify the conversion of a given device configuration to a position graph as suggested by Reviewer~2, we revised the caption of Figure \ref{fig:position_physical} with Reviewer~1's suggestion. Furthermore, we want to address this question by emphasizing that for a 2-dimensional QCCD-based TI device as defined in Section \ref{sec:QCCD}, where linear trap segments are connected through $X$- and $Y$- junctions, we explicitly show how to encode those in Section \ref{sec:ti_encoding} comprised with Figure \ref{fig:position_physical}. Moreover, to show that compilation on this abstraction is correct and sound, we show how the state of the position graph corresponds to the constraint of the QCCD device as described in Section \ref{sec:QCCD}. As a concrete example, Figure \ref{fig:state_of_position} shows how the state of position graph captures the constraints and movement of ions on the real device. Therefore, by dealing with the position graph state with our proposed heuristic as in Section \ref{sec:our_algo}, we are confident in the correctness and soundness of this compilation. \\

\noindent\textbf{Theoretical Evaluation:}\textit{``Poor''}

$\rightarrow$ As the main target of our paper is to propose a heuristic method to solve the shuttling problem. The theory part in this part is limited, but we have already added this up through the connection with the Token Reconfiguration problem and the formulation of MILP. We hope the changes make our theoretical aspect stronger.  \\

\noindent\textbf{Experimental Evaluation:} \textit{``The author evaluated SHARPER/SHAW on different QAOA applications and architectures. However, a more detailed explanation on why sometimes SHAW, the simpler heuristic method, performs better. The author should also evaluate or theoretical analysis the scalability of the method.''} 

$\rightarrow$ As describe in Section \ref{sec:PAS_and_PAM}, both of our proposed methods: SHAPER and SHAW, are heuristics that depend on some seed (initial ion assignment, synthesis seed, $\dots$). Therefore, the result of these heuristics can be different for different seeds. In our table, we only show the best result for each algorithm from 5 different seeds. Hence, randomness can be the case that makes SHAW better than SHAPER. 

For the evaluation of the scalability, we address this comment, as in the first part about the scalability concern ``\textbf{Question about the scalability of the proposed algorithms }''.\\

\noindent\textbf{Comparison with related state-of-the-art approaches:}\textit{``Comparsion with QCCDSim and integer programming is extensive, but cases with more qubits would be more appealing. Moreover, the author should compare to existing qubit mappers on superconducting devices, as the author claim the position graph can extend to superconducting quantum computers.''}

$\rightarrow$ Thank you for this comment. As described in our method Section \ref{sec:our_algo}, both the proposed SHAPER and SHAW are based on the PAM paper [arXiv.2305.02939], which is inspired by the SABRE algorithm. Rigorously, as shown in Appendix \ref{app:generalization_sc}, when considering the superconducting qubit system, our position graph abstraction makes the proposed evaluation of cost as defined in Equation \ref{eq:H} reduce to the original SABRE objective [arXiv.1809.02573]. Therefore, even with the use of position graph abstraction, when considering superconducting architecture, our proposed SHAPER is mapped back to PAM, and SHAW is mapped back to SABRE. Hence, we do not perform the numerical evaluation for the superconducting system, and the reviewer can find the performance of PAM and SABRE in the corresponding [arXiv.2305.02939, arXiv.1809.02573].\\

\noindent \textbf{Reasons to accept/reject:}
\begin{itemize}
    \item \textit{``The position graph abstraction is novel and practical for shuttling TI devices''}\\
    $\rightarrow$ Thank you for this comment
    \item \textit{``The author lacks a more vivid illustration of the position graph abstraction, including how it is corresponds to concrete actions on the devices, and why compilation on this abstraction is correct and sound''}\\
    $\rightarrow$ We hope our response can satisfy your concern. If there is any problem with the Figures that we use to illustrate the QCCD system and position graph, or if the conversion does not persuade you in any way. Please let us know, and we can make it clearer.
    \item \textit{``The SHARPER/SHAW compilers are efficient in compiling quantum circuits to shuttling TI devices with short shuttling time, and works when traditional methods failed to solve the scheduling''}\\
    $\rightarrow$ Thank you for your comment.
    \item \textit{``The paper lacks discussion on the scalability of both methods, only runtime cost are provided with small number of qubits.''}\\
    $\rightarrow$ We hope our response can satisfy your concern.
\end{itemize}


\subsection*{{Reviewer 3  comments: }}
\noindent\textbf{Novelty:} \textit{``The Position Graph abstraction is a significant conceptual merit of the paper, and the authors explain how this abstraction can be used to cast problems of routing and gate scheduling in trapped ions systems.''}

$\rightarrow$ Thank you for your comment.\\

\noindent\textbf{Soundness of the idea, and the methods and techniques proposed:} \textit{``The abstraction and the algorithms introduced to solve the shuttling problem in trapped ion machines are sound. However, the exact details of how to cast the shuttling problem into a Token Reconfiguration problem via the position graph are unclear and should be more thoroughly defined.''}

$\rightarrow$ Thanks for your question about the reduction of our problem to the Token Reconfiguration problem (TRP). To address this, we add more details to this part; the modification can be found in the second and third paragraphs in Section \ref{sec:theoretical_foundation_pg}.\\

\noindent\textbf{Experimental/Theoretical Evaluation:} \textit{``Benchmarks are comprehensive covering standard circuits from literature. The theoretical evaluation is also valuable with a clear connection to the Token Reconfiguration problem, pointing us to the complexity class of the problem the authors are attempting to solve.''}

$\rightarrow$ Thank you so much for your comment.\\

\noindent\textbf{Comparison with related state-of-the-art approaches:} \textit{``There is a direct comparison on multiple tasks with QCCDSim a state-of-the-art tool for the shuttling problem in trapped ion systems. The authors explain any patters in the results, including certain cases where QCCDSim outperforms SHAPER.''}

$\rightarrow$ Thank you so much for your comment.\\

\noindent\textbf{Presentation:} \textit{``Some definitions overload notions from related fields: e.g., "logical qubits" from quantum error correction (QEC) compared to this manuscript where they represent program qubits (closer to "physical qubits" from QEC). Additionally in Table 2, "ions/trap" which implies higher difficulty of the problem; in reality it means trap capacity, i.e., a lower level of difficulty as the "ions/trap" value increases. Moreover, the explanation of the graph reduction in Section 5.4 lacks the clarity needed to immediately distinguish it from standard TRP.''}

$\rightarrow$  Thanks for your comment on these notations. We agree with your comment and have modified those correspondingly by changing ``logical qubits'' to ``program qubits'' and changing ``ion/trap'' to ``trap capacity'' throughout the text. We hope the added details in Section \ref{sec:theoretical_foundation_pg} make it clear how to distinguish the Shuttling problem from the standard TRP.\\

\noindent\textbf{Reason to accept/reject:} \textit{
\begin{itemize}
    \item Terminology Overload: "logical qubits", which in this manuscript are closer to program qubits, creates confusion for the Quantum Error Correction community.
    \item The "reduction" in section 5.4 isn't direct from TRP requiring some intermediary generalized problems. The text should be more explicit on those problems, how the connection is done, and thus show how one adapts the TRP solver to the problem at hand.
    \item Legibility is a concern, with the most misleading part being the "Ions/Trap" column label in Tables 2. It should be immediately obvious why the larger number in this column represents the easier problem. An alternative would be trap capacity or some clarification in the table's caption.
\end{itemize}}

$\rightarrow$ Thanks for all the concern that you have shown. These really help improve the manuscript by a lot. We hope all of our answers can satisfy your concern.\\

\noindent\textbf{Additional comments:} \textit{``It is slightly misleading that the introduction and section 4 recognize heating as a culprit for lowered circuit fidelities, but SHAPER and SHAW optimize for runtime. Yes, to first order lowered runtime implies lowered heating, but as the authors note in section 8, certain ions are more prone to heating dependent on how much they are moving, what type of junctions they traverse, etc.''}

$\rightarrow$ To address this, we first clarify the relationship between operation runtime, heating, and the fidelity model by clarifying it through the modification in the Section \ref{sec:Intro}: Introduction and Section \ref{sec:QCCD}. Moreover, the details about the fidelity model are discussed in Section \ref{sec:exp_setup}.\\

\noindent\textit{``Another issue is the number of dummy nodes from the appendices. This number isn't clearly defined and raises issues with regards
''}

$\rightarrow$ For the comment about the number of dummy nodes, we clarify it by adding a concrete example related to our experiment in Appendix \ref{sec:shuttling_MILP}
\newpage

==> isca2024/content/rebuttal_letter_2.tex <==
\newpage
\section*{Author's response letter}
Dear Reviewers and Editors,

We express our gratitude to all reviewers for their time and effort. The comments are absolutely invaluable and helped to improve the paper. Especially, we thank Reviewer~1 and Reviewer~3 for accepting the manuscript, and Reviewer~2 for some valid concerns that strengthened the paper after revision. In this revision, we mainly address Reviewer~2's comments by performing an update on the current codebase, which allows better timing and better compilation performance. In this revision, we have implemented many modifications and clarifications that enhance the quality of the manuscript according to the reviews.

\begin{itemize}
    \item Reviewer~1's comment about the table format: We have fixed the scaling of every Table inside the manuscript
\end{itemize}

New content has been highlighted in \color{blue} Blue \color{black} in the revised manuscript for easy identification.\\


\noindent\textbf{Issues (1) :} \textit{The authors mention that alternative graph algorithms with lower complexity than the Floyd – Warshall algorithm could be considered. However, such alternatives have not been implemented or evaluated.} \\


$\rightarrow$ Here, we want to clarify that for both SHAW and SHAPER, given a fixed architecture, the Floyd–Warshall algorithm can be engineered to be run only once during the compilation process over multiple benchmarks. Therefore, the algorithm overhead is not big on the current graph scale. The current experiments are carried out around a $200$-node position graph abstraction, and even when going to $1000$-node graphs, as shown in \cite{brent2026scaling}, it is not the main issue for the timing. Therefore, we do not implement or evaluate other alternatives. To be more specific, the Floyd–Warshall algorithm takes $0.00405$ seconds for the G$6\times6$ architecture with trap capacity of $5$, and takes $0.25$ seconds for the G$13\times 13$ architecture with trap capacity of $8$.\\


\noindent\textbf{Issues (2) :} \textit{A scalability analysis based on the model $y = ax^b$ (where x is the number of ions) has been provided. However, lower asymptotic complexity does not necessarily translate into practical efficiency, and thus the argument remains only partially convincing.}

$\rightarrow$ We thank the reviewer for the correct concern about the practicality of the compilation runtime. Even though we have a competitive asymptotic complexity from the last experiments, this can indeed still lead to practical inefficiency. Here, to address this comment while still having a fair comparison with QCCDSim, we perform code refactoring on all methods to ensure a competitive compilation runtime for all methods. Furthermore, we use the University of Delaware cluster system with the following settings: 32-core AMD EPYC 7702 processor with 1TB of memory, to re-benchmark the current results. Here, as a result of the engineering process, we obtain a big improvement in compilation runtime over all benchmarks compared to the last manuscript, which can be seen in Tables 3 and 5. Furthermore, in our latest work \cite{brent2026scaling}, we enhance the current method with memoization and a pruning method similar to \cite{zou2024lightsabre}, which enhances the scaling of our technique further. In \cite{brent2026scaling}, we scale up the experiments to $1024$-qubit circuits with an architecture configuration of G$13\times13$ and a trap capacity of $8$, showing a significant improvement in compilation time compared with QCCDSim. At the same time, it always yields a better total operation time, comprised of shuttling time and gate execution time.
\\


\noindent \textbf{Unresolved critical concern (1):} 
\textit{
The proposed methods incur far higher compile time (several orders of magnitude greater) over prior work, and do not consistently demonstrate improved fidelities. This compilation overhead issue (also raised in the first review) has not been sufficiently addressed and is also observed in the large-scale experiments (newly added in the revised version). The authors analyze runtime scaling using the model $y = ax^b$, where $x$ denotes the number of ions inside the architectures. While the exponent for SHAPER and SHAW is approximately 3, compared to approximately 6 for QCCDSim, suggesting a quadratic improvement in asymptotic scaling. However, the constant factor remains worse. Algorithms with better asymptotic complexity are not always preferable in practice. For example, in Table 5, for the QAOA\_32 benchmark on a G3x3 architecture (9 traps, trap capacity = 5), QCCDSim
requires 1.367 seconds of compilation time and produces a schedule with an operation time of 67 ms. In contrast,
SHAPER requires 1170.82 seconds of compilation time while reducing the operation time to 44 ms. Similarly, for the
QAOA\_128 benchmark on a G6x6 architecture (36 traps, trap capacity = 5), QCCDSim completes compilation in
approximately 1 minute and 36 seconds, yielding an operation time of 0.8 seconds. In contrast, SHAPER requires
nearly a full day of compilation time to reduce the operation time to 0.4 seconds.
Even under very conservative assumptions about hardware scaling from the late NISQ era to early FTQC systems,
such compile-time versus runtime trade-offs remain difficult to justify. This is because the TI runtime constitutes only
a small fraction of the overall execution pipeline; from the perspective of Amdahl’s law, improvements in this
component alone are unlikely to translate into substantial end-to-end gains. For the current manuscript to be
convincing, it is therefore necessary to provide a compelling justification for why such significant compilation
overhead is warranted.
}

$\rightarrow$ We thank the reviewer for pointing out the important distinction between asymptotic complexity, compilation runtime, and schedule quality. We agree that a compiler with a higher classical runtime is not universally preferable. As mentioned in the above answer, we have added the engineering process to optimize our code, which leads to faster compilation runtime. Specifically, for QAOA\_32 benchmark on a G3x3 architecture (9 traps, trap capacity = 5), QCCDSim now requires 0.09 seconds of compilation time while SHAW now only requires $78.6$ seconds, which is a $15$ times reduction. The operation time remains the same, where QCCDSim's schedule takes 67 ms, and SHAW's schedule takes 44 ms. Similarly, for the QAOA\_128 benchmark on a G6x6 architecture (36 traps, trap capacity = 5), QCCDSim now requires 2 minutes and 4 seconds, resulting in an operation time of 0.8 seconds. In contrast, SHAPER requires 10 hours of compilation time to reduce the operation time to 0.35 seconds.

Second, we want to emphasize the importance of operations time and have revised the discussion to make this trade-off explicit. In the QCCD setting, the two quantities compared by the reviewer have different operational roles: compilation is an offline classical preprocessing cost, whereas the reported operation time is an online hardware execution cost paid every time the circuit is run. This distinction is especially important for quantum algorithms because a single execution shot of a quantum circuit only produces one sample. Most meaningful quantum algorithmic outputs, such as expectation values, objective estimates, or output distributions, require repeated circuit executions over many shots and often over many parameter evaluations in hybrid algorithms such as QAOA. As concrete examples, \cite{kotil2025quantum} performs multi-objective QAOA, where $25$ million shots were taken in total; \cite{farrell2024quantum} performs quantum simulation on IBM’s 133-qubit Heron processor with $154$ million shots, and \cite{hempel2018quantum} performs VQE on Trapped-ion devices where each experiment requires $15k$ shots.


Therefore, a reduction in operation time can be amortized over repeated executions of the same compiled circuit. Moreover, in shuttling-based trapped-ion systems, operation time is not merely a throughput metric. Prior experimental work reports that immense shuttling introduces heating, which excites ion motion during QCCD computation, requiring cooling to maintain high-fidelity gate performance. QCCD operation time is strongly affected by ion transport: shuttling can consume a significant fraction of the total algorithm time, and motional excitation during shuttling can reduce the fidelity of entangling gates \cite{sterk2022closed}. Thus, shorter schedules can improve both online throughput and reliability, while longer schedules increase exposure to shuttling-induced heating, cooling overhead, and fidelity loss \cite{fallek2024rapid, kaushal2020shuttling}. Furthermore, the economic comparison also favors reducing online operation time. Suppose an improved compiler requires 10 additional CPU-hours. At a representative cloud CPU price of $\$0.18$/hour, this costs about $\$1.80$. If the resulting schedule saves only $0.01$ seconds of QPU time per shot, then over $10^6$ shots it saves $10,000$ seconds of online QPU time (which costs much more than $\$1.80$). On any time-metered QPU service, this online saving is far larger than the few-dollar offline CPU cost. More information on the pricing of QPU can be found on the IBM and AWS Bracket website, but the cost can be up to $\$96$/minute.


To clarify this trade-off, we added an amortized break-even analysis here with the latest results from Table 5. For example, on QAOA\_32 with G3x3 and trap capacity 5, SHAW reduces the operation time from 67.066 ms to 38.871 ms with an additional compilation cost of 78.51 s compared to QCCDSim, giving a break-even point of approximately 2.8k circuit shots. For QAOA\_128 with G6x6 and trap capacity 5, SHAW reduces operation time from 795.877 ms to 356.547 ms, with a break-even point of approximately 82k circuit shots. Thus, QCCDSim can be preferable for a one-shot sample when it succeeds, while SHAW/SHAPER becomes preferable in repeated execution or fidelity-sensitive settings


% This compile-time/operation-time trade-off is also relevant to future fault-tolerant trapped-ion compilation. Although our present compiler does not directly optimize encoded logical circuits or syndrome-extraction schedules (physical compilation), it addresses the same underlying physical bottleneck: online operation time on a shuttling-based QCCD architecture through logical compilation. QEC requires cyclic syndrome extraction throughout the computation, and fault-tolerant resource estimates show that total runtime is highly sensitive to code-cycle time and scheduling overhead~\cite{battistel2023real}. For example, prior estimates give 8 hours for RSA-2048 factoring with 20 million noisy qubits under a $1\,\mu$s surface-code cycle \cite{gidney2021factor}, under 4 days for FeMoCo simulation with about four million physical qubits under similar assumptions, and thousands of days for a shuttling-based trapped-ion FeMoCo estimate without sufficient parallelization\cite{webber2022impact}. 

% These results motivate future QEC-aware extensions of the position graph abstraction, where reducing shuttling and online schedule length could directly reduce the cost of repeated syndrome extraction and logical operations. \\


Currently, our compilation algorithm optimizes logical operations at the program level and doesn't consider the physical layer of quantum error correction (QEC). While we do not directly handle syndrome extraction, decoding, or magic-state factories, the methods proposed here can potentially be adapted to future fault-tolerant pipelines. When translating from logical to physical circuits, milliseconds can become hours. For example, Gidney and Eker{\aa} estimate RSA-2048 factoring using about 20 million noisy physical qubits and roughly 8 hours of runtime under a $1\,\mu$s surface-code cycle, while Lee et al. estimate FeMoCo simulation using about four million physical qubits and under four days of runtime under similar code-cycle assumptions~\cite{gidney2021factor,lee2021even}. In this high-overhead environment, logical delays act as a multiplier. By shaving milliseconds off a logical schedule, a compiler can potentially trim hours or even days from the final physical execution.


% This compile-time/operation-time trade-off is also relevant to future fault-tolerant trapped-ion compilation, but we emphasize the distinction between logical/application-level compilation and physical/QEC-level compilation. The present work operates at the program circuit level: it maps and schedules unencoded circuit operations on a shuttling-based QCCD architecture, and it does not directly compile the full physical implementation of an encoded computation, including syndrome extraction, decoding, lattice surgery, or magic-state factories. The fault-tolerant resource estimates, therefore, illustrate how savings in online logical schedule length can be amplified after QEC expansion. For example, Gidney and Eker{\aa} estimate RSA-2048 factoring using about 20 million noisy physical qubits and roughly 8 hours of runtime under a $1\,\mu$s surface-code cycle, while Lee et al. estimate FeMoCo simulation using about four million physical qubits and under four days of runtime under similar code-cycle assumptions~\cite{gidney2021factor,lee2021even}. These millions of qubits are physical qubits after QEC expansion, not the number of program qubits that our compiler must handle directly. Thus, while our current position-graph compiler is not a physical QEC compiler, reducing online QCCD operation time at the logical scheduling layer provides a concrete foundation for future QEC-aware compilation, where even millisecond-level savings in repeated logical schedules may translate into substantial reductions (days) in physical runtime after error-correction overheads are included.

% We have therefore clarified that SHAPER/SHAW should be interpreted as occupying a different point in the compile-time/operation-time Pareto frontier. QCCDSim is attractive when a one-shot compilation is needed, and it succeeds. SHAPER/SHAW are preferable in repeated-execution, high-utilization, or fidelity-sensitive regimes, where online execution time and shuttling-induced reliability effects dominate the one-time offline compilation cost.

\noindent\textbf{Unresolved critical concern (2):} \textit{This reviewer believes that such justification should come from clear and consistent improvements in computational accuracy, namely circuit fidelity. Unfortunately, the results in Table 4 indicate that the proposed methods achieve consistently higher fidelity than QCCDSim only for small (8-qubit) workloads. Fidelity improvements are not consistently observed. For instance, under the QFT\_16 benchmark on a G2x3 architecture (6
traps, trap capacity = 4), SHAPER yields 4.43× lower fidelity and SHAW yields 12× lower fidelity compared to
QCCDSim. These results weaken the argument for adopting the proposed methods, even when substantially longer
compilation times are tolerated.}

$\rightarrow$ We thank the reviewer for the valid concern. However, we want to emphasize that while the operation time (shuttling time) can not fully describe the circuit fidelity objective, the heating introduced by long operation time is still the main factor. Therefore, most experimental papers point out the need to minimize the shuttling time. This is indeed true with the current fidelity model, where substantially better operation time always leads to better fidelity. Indeed, the main reason for the fall in fidelity for the SHAPER and SHAW in the last results is due to comparable operation times. Therefore, to address these performance concerns, we did two things

First, we re-run the experiments for small to medium-sized circuits with more passes (4 passes) to ensure a better operation time schedule that always results in much better operation time, as shown in Table 3. This leads to much better fidelity results, as shown in Table 4. Consequently, we also modify the discussion on the fidelity result in the paragraph \textit{Gate count overhead and Circuit fidelity} in Section 7.2. We also want to note that for bigger cases ($32$ to $128$-qubit circuits), our schedules, as having a very big gap in operation time, always yield better fidelity compared to QCCDSim.


% \blue{Furthermore, to have a synthesis objective well-tailored to circuit fidelity, the characteristic of the considered fidelity model can be incorporated. As a concrete example, the fidelity model in Section \ref{sec:exp_setup} gets worse when one ion is involved in many gate operations, as it potentially carries more heating, which leads to worse gate fidelity. Therefore, the synthesis objective can also try to balance the number of gates that act across ions along with gate counts and congestion.}

Second, the fidelity illustrated is through a fidelity model, which also does not fully capture the dynamics of a real QCCD system. Different fidelity models may emphasize different physical effects, such as accumulated motional excitation, ion-dependent heating, cooling overhead, or gate-specific error rates. Therefore, our compiler can, in principle, exploit the structure of a given fidelity model to produce schedules that are better with respect to that model.
 
As a concrete example, in the fidelity model used in Section~7.1, an ion that participates in many gate operations may accumulate more heating, which leads to lower gate fidelity. This suggests that the synthesis or routing objective can be modified to balance the number of gates acting on each ion, in addition to minimizing gate count, congestion, and shuttling time. We observed that this type of model-aware objective can improve the schedule fidelity under the specific fidelity model considered in this paper. However, we also recognize that such improvements should not be interpreted as universal hardware-level fidelity gains. Without a hardware-calibrated fidelity model, aggressively optimizing for a particular analytic model risks overfitting to the assumptions of that model rather than improving performance on a real device. For this reason, we add a paragraph in the Discussion about this approach for future work shown in Section 8, paragraph \textit{Toward fidelity-aware position-graph compilation}. \\


\noindent\textbf{Constructive suggestions from Reviewer~2} \textit{Despite the above concern, this reviewer would like to offer constructive suggestions that may help the work meet the TQC bar: If lighter-weight graph algorithms than Floyd–Warshall are indeed applicable, could the authors implement and evaluate such alternatives to reduce compilation overhead?}

$\rightarrow$ The author answered this question in the first \textbf{Issues (1)}.\\


\textit{Moreover, although the revised circuit
synthesis considers both gate count and shuttling, but fidelity is not consistently improved. As noted by the authors near Equation 4, motion, and heating are key factors affecting fidelity. Incorporating these factors directly into the synthesis objective may further improve fidelity outcomes. Overall, even if the proposed methods achieve fewer wins in terms of the operation time, they could become competitive with QCCDSim if they provide (i) consistent fidelity improvements and (ii) reduced compilation overhead compared to the current implementation.}

$\rightarrow$ We thank the Reviewer for constructive feedback. For the revised version, we now ensure consistent fidelity improvements, as shown in the answer to \textbf{Unresolved critical concern (2):} and we perform code refactoring to reduce compilation overhead, as shown in the answer in \textbf{Issues (2)}.\\


\textit{Additionally, this reviewer suggests that it may be helpful to emphasize that circuit synthesis need not be repeated for every execution once a hardware architecture is provided. This might strengthen the argument that the proposed approach can
justify far higher compilation overhead in exchange for improved fidelity and QPU runtime. Still, please check that this argument makes sense.}

$\rightarrow$ We thank the Reviewer for the suggestion. However, circuit synthesis needs to be performed for different circuits with respect to different architectures. Each circuit only needs to be synthesized once for each architecture, and the mapping and shuttling process happens. 
